The Lernaean Hydra of Data Series Similarity Search: An Experimental Evaluation of the State of the Art

Increasingly large data series collections are becoming commonplace across many different domains and applications. A key operation in the analysis of data series collections is similarity search, which has attracted lots of attention and effort over the past two decades. Even though several relevant approaches have been proposed in the literature, none of the existing studies provides a detailed evaluation against the available alternatives. The lack of comparative results is further exacerbated by the non-standard use of terminology, which has led to confusion and misconceptions. In this paper, we provide definitions for the different flavors of similarity search that have been studied in the past, and present the first systematic experimental evaluation of the efficiency of data series similarity search techniques. Based on the experimental results, we describe the strengths and weaknesses of each approach and give recommendations for the best approach to use under typical use cases. Finally, by identifying the shortcomings of each method, our findings lay the ground for solid further developments in the field.

==> intro.bup.tex <==
\section{Introduction}
\label{sec:introduction}
\noindent{\bf Data Series.}
A data series is an ordered sequence of data points\footnote{When the sequence is ordered on time, it is called a \emph{time series}.
However, the order can be defined by angle (e.g., in radial profiles), mass (e.g., in mass spectroscopy), position (e.g., in genome sequences), and others~\cite{conf/sofsem/Palpanas2016}. The terms \emph{data series}, \emph{time series} and \emph{sequence} are used interchangeably.}.
Data series are one of the most common types of data, covering virtually every scientific and social domain, such as astrophysics, neuroscience, seismology, environmental monitoring, biology, health care, energy, finance, criminology, social studies, video and audio recordings, and many others~\cite{KashinoSM99,Shasha99,humanbehaviorpatterns,volker,DBLP:conf/edbt/MirylenkaCPPM16,HuijseEPPZ14,percomJournal,windturbines,spikesorting,VALMOD,journal/jte/Williams2003,conf/compstats/Hebrail2000}.
As more devices, applications, and users are connected with IoT technologies, an increasingly large number of data series is generated, leading to multi-TB collections~\cite{DBLP:journal/sigmod/Palpanas15}.
We note that, when these collections are analyzed, the common denominator of most analysis algorithms and machine learning methods, e.g., outlier detection~\cite{journal/csur/Chandola2009,journal/vldb/Dallachiesa2014}, frequent pattern mining~\cite{conf/kdd/Mueen2012}, clustering~\cite{conf/kdd/Keogh1998,conf/sdm/Rodrigues2006,conf/icdm/Keogh2011, journal/pattrecog/Warren2005}, and classification~\cite{journal/jmlr/Chen2009}, is that they are based on similarity search.
That is, they require to compute distances among data series, and this operation is repeated many times.

\noindent{\bf Data Series Similarity Search.}
Similarity search is the operation of finding the set of data series in a collection, which is close to a given query series according to some definition of distance (or similarity).
A key observation is that similarity search needs to process a sequence (or subsequence) of values as a single object, rather than as individual, independent points, which is what makes the management and analysis of data sequences a hard problem with a considerable cost.
Therefore, improving the performance of similarity search can improve the scalability of data analysis algorithms for massive data series collections.

Nevertheless, despite the significance of data series similarity search, and the abundance of relevant methods that have been proposed in the past two decades~\cite{conf/fodo/Agrawal1993, conf/vldb/Ciaccia1997,conf/kdd/shieh1998, conf/icde/Rafiei99, conf/kdd/ColeSZ05, conf/icdm/Camerra2010, conf/kdd/Karras2011, conf/kdd/Mueen2012,journal/edbt/Schafer2012,conf/vldb/Wang2013, journal/kais/Camerra2014,journal/vldb/Zoumpatianos2016, code/Mueen2017,dpisax,ulisse,journal/vldb/linardi18,conf/bigdata/peng18}, no study has ever attempted to compare these methods under the same conditions. 
We also point out that we focus on the \emph{efficiency} of similarity search methods, whereas previous works studied the \emph{accuracy} of dimensionality reduction techniques and similarity measures, focusing on classification~\cite{journal/dmkd/Keogh2003, conf/vldb/Ding2008, DBLP:journals/datamine/BagnallLBLK17}. 

In this experimental and analysis paper, we thoroughly assess different data series similarity search methods, in order to lay a solid ground for future research developments in the field.
In particular, we focus on the problem of \emph{exact whole matching similarity search in collections with a very large number of data series}, i.e., similarity search that produces exact (not approximate) results, by calculating distances on the whole (not a sub-) sequence.
This problem represents a common use case across many domains~\cite{url:adhd,url:sds,conf/compstats/Hebrail2000,SENTINEL-2}. 
This work is the most extensive experimental comparison of the efficiency of 
similarity search methods ever conducted. 
\noindent{\bf Contributions.}
We make the following contributions:
1. We present a thorough discussion of the data series similarity search problem, formally defining its different variations that have been studied in the literature under diverse and conflicting names. Thus, establishing a common language that will facilitate further work in this area.
2. We include a brief survey of data series similarity search approaches, bringing together studies presented in different communities that have been treated in isolation from each other.
These approaches range from smart serial scan methods to the use of indexing, and are based on a variety of classic and specialized data summarization techniques.
3. We make sure that all approaches are evaluated under the same conditions, so as to guard against implementation bias.
To this effect, we used implementations in C/C++ for all approaches, and reimplemented in C the ones that were only available in other programming languages. Moreover, we conducted a careful inspection of the code bases, and applied to all of them the same set of optimizations (e.g., with respect to memory management, Euclidean distance calculation, etc.), leading to considerably faster performance.
4. We conduct the first comprehensive experimental evaluation of the efficiency of data series similarity search approaches, using several synthetic and 4 real datasets from diverse domains.
In addition, we report the first large scale experiments with carefully crafted query workloads that include queries of varying difficulty, which can effectively stress-test all the approaches.
Our results reveal characteristics that have not been reported in the literature, and lead to a deep understanding of the different approaches and their performance.
Based on those, we provide recommendations for the best approach to use under typical use cases, and identify promising future research directions.
5. We make available online all source codes, datasets, and query workloads used in our study~\cite{url/DSSeval}. 
This will render our work reproducible and further help the community to agree on and establish a much needed data series similarity search benchmark~\cite{journal/dmkd/Keogh2003, conf/kdd/Zoumpatianos2015, johannesjoural2018}.

